On the Convergence of No-Regret Dynamics in Information Retrieval Games with Proportional Ranking Functions

Publishers who publish their content on the web act strategically, in a behavior that can be modeled within the online learning framework. Regret, a central concept in machine learning, serves as a canonical measure for assessing the performance of learning agents within this framework. We prove that any proportional content ranking function with a concave activation function induces games in which no-regret learning dynamics converge. Moreover, for proportional ranking functions, we prove the equivalence of the concavity of the activation function, the social concavity of the induced games and the concavity of the induced games. We also study the empirical trade-offs between publishers' and users' welfare, under different choices of the activation function, using a state-of-the-art no-regret dynamics algorithm. Furthermore, we demonstrate how the choice of the ranking function and changes in the ecosystem structure affect these welfare measures, as well as the dynamics' convergence rate.

==> OlderVersions/NeurIPS_2024/backup.tex <==
% Importantly, although we use discrete uniform distributions, in a random selection of the support this distribution can induce games with strategic characteristics similar to other distributions. This is due to the continuity of the ranking functions. 
% For example, you can look at a simple non-uniform distribution where \(P^*(x^*_1)=\frac{2}{3}\) and \(P^*(x^*_2)=\frac{1}{3}\). If we take a discrete uniform distribution \(s=3\) where \(x^*_1\) and \(x^*_2\) are relatively close points and \(x^*_3\) is in another area we will get a similar strategic behavior of the publishers because the values of the ranking functions for the two distributions will be relatively close almost everywhere.
% Note that any distribution can be approximated by a uniform distribution if \(s\) is big enough. Appendix ??? discusses big values of \(s\).


%--------------------------------



% \footnote{When comparing the $\lambda$ values we could use the same random set of initial documents and demand function's support constant for different $\lambda$ values, but this is not possible when considering other parameters accordingly the results we got are less stable.}




%--------------------------------



% \subsection{Regret comparison}

% \begin{figure}
% \centering
% \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{static_figures/regret_rounds.png}
% \caption{The sum of the regret of the publishers in an example instance with $\lambda=0.5, n=3, k=3$ and $s=3.$ For all publishers, the difference between the total regret at round $100$ and $1000$ is smaller then $10^{-5}$.}
% \label{fig: regret rounds}
% \end{figure}

% \paragraph{Measuring regret} An important feature of the dynamics is the total regret of the publishers. In order to compare the regret of the publishers with different ranking functions and game parameters we run a slightly different kind of simulations. In order to keep the comparison unbiased, in those simulation we simulate a constant number of rounds each time and calculate the regret across the dynamics for each publisher and divide it by the number of rounds. We chose to run each simulation for $100$ rounds due to the fact that we saw that the total regret of the player in the $100$ first rounds almost exactly approximates the regret he will have over a large number of rounds. Figure \ref{fig: regret rounds} present the increase in the cumulative regret of each player at an example instance. It can be seen from the Figure the the regret at round $100$ approximates almost exactly the cumulative regret of the publishers, therefore we can use the average regret of the first $100$ rounds on order to compare the regret under different ranking functions and game parameters.

% אולי להסביר למה 100 זה מספיק כדי להשוואות - רוב הסימולציות מתכנסות בהרבה פחות וגם מהתרשים ברור שהחרטה כבר לא תגדל הרבה, גם אני נריץ עד ל10000

% \begin{figure}
% \centering
% \includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{static_figures/regret_graphs_exemple.png}
% \caption{The effects of $\lambda, n, k$ and $s$ on the average regret of the publishers. The base parameters values are: $\lambda = 0.5, n = 3, k = 3$ and $s = 3$}
% \label{fig: regret comp}
% \end{figure}

%You: צריך לתת שם שונה לחרטה ממוצעת לכל שחקן ולחרטה ממוצעת של כל השחקנים

% \paragraph{Regret comparison}
% Figure \ref{fig: regret comp} present the effect of different ranking functions and game parameters on the regret. 
% TODO: difference and correlation between the regret trends and the convergence rate trends

==> OlderVersions/abstract.tex <==
Publishers who publish their content on the web act strategically, in a behavior that can be modeled within the online learning framework. 
Regret, a central concept in machine learning, serves as a canonical measure for assessing the performance of learning agents within this framework.
We prove that any proportional content ranking function with a concave activation function induces games in which no-regret learning dynamics converge. 
Moreover, for proportional ranking functions, we prove the equivalence of the concavity of the activation function, the social concavity of the induced games and the concavity of the induced games.
We also study the empirical trade-offs between publishers' and users' welfare, under different choices of the activation function, using a state-of-the-art no-regret dynamics algorithm. Furthermore, we demonstrate how the choice of the ranking function and changes in the ecosystem structure affect these welfare measures, as well as the dynamics' convergence rate.

==> OlderVersions/body.tex <==
\section{Introduction}

In the era of digital content consumption, recommender systems play an essential role in shaping user experiences and engagement on various platforms, including search engines, streaming services, social networks, and more. The core task of a recommender system is to match users with relevant content, created by content creators. By that, the system induces an ecosystem in which content providers compete for exposure and often engage in strategic behavior to maximize visibility \cite{qian2024digital}. In particular, the specific recommendation mechanism used by the platform determines the incentives, and hence the strategic behavior, of the content providers. In the context of search engines, this phenomenon is often referred to as \emph{Search Engine Optimization (SEO)} and is widely observed in real-world search engines \cite{compSearch}.

These dynamics have major implications for various economic aspects of the ecosystem. First, strategic behavior affects the \emph{welfare} of both end users (seeking relevant content) and content creators, whose profits are often proportional to the level of exposure they receive from the platform. The second aspect is \emph{stability}, which refers to the existence of, and the convergence to, a stable state, in which content providers have no incentive to modify their content given the content provided by their competitors. In the game-theoretic jargon, this stability is captured by the notion of \emph{Nash equilibrium}. Not surprisingly, these two aspects have been shown, for example empirically in \cite{madmon2024search}, to be interconnected. 

The study of convergence to equilibrium through the lens of game theory, a field often referred to as \emph{learning dynamics}, has been adopted to analyze the stability of recommendation and ranking mechanisms. Specifically, two concrete dynamics that arise in the presence of strategic behavior over time are \emph{better-response dynamics} and \emph{no-regret dynamics}.
The convergence of better-response dynamics has been studied in the context of information retrieval under different modeling assumptions \cite{ben2019convergence,madmon2024search}. In this paper, we study no-regret learning dynamics in information retrieval games. We adopt the game-theoretic framework of \cite{yao2024rethinking,madmon2024search}, in which both content and users are represented in a continuous, multi-dimensional embedding space, and the content providers aim to maximize exposure while maintaining the integrity of their original content. As in \cite{madmon2024search}, and unlike in \cite{yao2024rethinking}, we consider mechanisms that only control the exposure of each content provider, without any additional reward in the form of payments (as done in platforms such as YouTube \cite{youtube}). These mechanisms contain, among others, search engines that control the probability of presenting documents in response to a user query. That is, the mechanism considered is a \emph{ranking function} which is a mapping from the publishers' documents to a distribution over the publishers, determining each publisher's exposure rate.


\paragraph{Our contribution} 
% We initiate the study of no-regret learning dynamics in information retrieval games. 
In the spirit of previous work \cite{hron2022modeling,jagadeesan2206supply,yao2024rethinking,madmon2024search}, we model SEO as a game and define a natural class of ranking functions we term \emph{proportional ranking functions}. While in our model a ranking function is a vector-valued function (as it assigns exposure probabilities for each publisher), a proportional ranking function is uniquely defined by a one-variable scalar function, which we call an \emph{activation function}. 
Importantly, the choice of the ranking function determines the incentives of the strategic publishers and hence affects the content available to users in the corpus. Relying on the notion of socially concave games, a subclass of concave games presented in \cite{10.1145/1536414.1536486}, we prove that the concavity of the activation function guarantees the convergence of any no-regret learning dynamics in any induced SEO game. 
To do so, we establish a rather stronger statement by proving the equivalence of the following three conditions: the activation function is concave; any induced game is socially-concave; any induced game is concave (as in \cite{rosen1965existence}). 
% Note that while in general any socially-concave games is concave and the opposite is not true, in our settings both directions hold.
We also study the empirical trade-offs between users' and publishers' welfare under different choices of the activation function, using a state-of-the-art no-regret dynamics algorithm \cite{Farina2022NearOptimalNL}. 
In addition, we demonstrate the effect of the game parameters such as the penalty factor and the number of publishers on the publishers' welfare, the users' welfare and the convergence rate.


\subsection{Related work}

In a recent growing line of research work, a variety of game-theoretic frameworks have been proposed to analyze the strategic dynamics of content providers in recommendation systems, particularly in the context of search engines. The study of strategic behavior of content creators under the mediation of a recommender system was initiated in a series of research works \cite{ben2017shapley,ben2018game,ben2019recommendation}. The Shapley mediator was proposed as a mechanism satisfying both stability (in the form of equilibrium existence guarantee) as well as fairness-related axioms. 

Another concurrent line of works focused on the analysis of an adversarial information retrieval framework, in which content providers compete on exposure \cite{ben2015probability,basat2017game}. These works demonstrated the sub-optimality of greedy ranking according to the probability ranking principle (PRP) of \cite{robertson1977probability} in terms of social welfare at equilibrium. \cite{raifer2017information} then studied both theoretically and empirically the SEO competition in a repeated setting. Under similar modeling assumptions, \cite{ben2019convergence} showed that better-response dynamics of publishers in PRP-based retrieval games are guaranteed to converge.

More recent studies on strategic behavior within recommendation and search ecosystems have adapted several modeling assumptions that reflect the use of deep learning and dense representations \cite{hron2022modeling,jagadeesan2206supply,yao2024rethinking,madmon2024search}. Unlike earlier studies, these recent efforts assume that content is represented within a continuous embedding space, rather than a discrete set of "topics". In contrast to \cite{yao2024rethinking}, we focus on the case in which the platform can only control the exposure rate of the publishers. The main focus of these works was on equilibria characterization \cite{hron2022modeling,jagadeesan2206supply} and the study of better-response dynamics convergence \cite{madmon2024search} under specific recommendation or ranking mechanisms. In contrast, this work characterizes a rich and intuitive family of mechanisms that guarantee the convergence of \emph{no-regret dynamics}.

The fundamental connections between no-regret learning and game-theoretic solution concepts \cite{foster1997calibrated,freund1999adaptive,hart2000simple,blum2008regret,roughgarden2015intrinsic} have made the regret-minimization framework very appealing to the machine learning and artificial intelligence communities \cite{rakhlin2013optimization,bowling2015heads,syrgkanis2015fast,moravvcik2017deepstack,brown2018superhuman,kangarshahi2018let,daskalakis2021near, Farina2022NearOptimalNL,anagnostides2024convergence}. In particular, the notion of concave games \cite{rosen1965existence} and its connection to the convergence of no-regret dynamics showed by \cite{10.1145/1536414.1536486} plays a crucial role in our analysis.


\section{Preliminaries}

\paragraph{Game theory} An $n$-person game is a tuple $G=(N, \set{X_i}_{i \in N}, \set{u_i}_{i \in N})$, where $N=\set{1,...,n}$ is the set of players, $X_i$ is the set of actions of player $i$, and $u_i: X \to \R$ is the utility function of player $i$, where $X = X_1 \times ... \times X_n$ is the set of all possible action profiles. Throughout the paper, we assume that for every player $i$, $X_i$ is a convex and compact set of actions. In addition, we assume that $u_i$ is twice differentiable and bounded for all $i$.

For any action profile $x \in X$, we denote by $x_{-i} = (x_1, ... x_{i-1}, x_{i+1} , ... x_n)$ the actions of all players except player $i$ within the profile $x$. An action profile \(x\) is said to be an \emph{$\varepsilon$-Nash equilibrium} ($\varepsilon$-NE) if for any player $i$, and for any action $x'_i \in X_i$, deviation of player $i$ from $x_i$ to $x'_i$ does not increase her utility by more than $\varepsilon$. Formally, 
for any $\varepsilon \ge 0$, \(x \in X\) is an \(\varepsilon\)-NE if \(u_i(x'_i, x_{-i}) - u_i(x) \le \varepsilon, \forall i \in N, \forall x'_i \in X_i\). For \(\varepsilon=0\), a \(0\)-NE is referred to as a \emph{Nash equilibrium} (NE).


% For \(\varepsilon = 0\), the set \({NE}(G) \coloneqq NE_0(G)\) is referred to as the set of Nash equilibria of the game \(G\).

\paragraph{No-regret dynamics} No-regret dynamics is a well-known type of dynamics within the \textit{online learning framework}, in which each player \(i\) is a learning agent that has to select a strategy \(x_i^{(t)} \in X_i\) in every round \(t \in \N\), in response to the sequence of the observations she has received up until round \(t\). A widely acceptable way to measure the performance of player \(i\) up to some horizon time \(T \in \N\) in this setting is \textit{regret},\footnote{We consider the notion of external regret, not to be confused with internal ('swap') regret.} defined as follows:

 \begin{equation}
     \text{Reg}^T_i \coloneqq \max_{x_i \in X_i} \Biggl \{\sum_{t=1}^{T} u_i(x_i, x_{-i}^{(t)}) \Biggr \} - \sum_{t=1}^T u_i(x^{(t)})
 \end{equation}

 That is, the regret of player \(i\) is measured with respect to the utility she could have gained had she selected in every round the best fixed strategy in hindsight. In our context, as standard in the online learning literature, e.g. \cite{Farina2022NearOptimalNL}, it is assumed that each player observes in every round \(t\) the gradient of her utility function with respect to her strategy, evaluated at the strategy profile selected by all players in this round. That is, in round \(t\) player \(i\) observes \(\nabla_{x_i} u_i (x^{(t)})\).

\paragraph{Concave games} We now introduce two special classes of games. A game $G$ is said to be a \emph{(strictly) concave game} if for any player $i$, $u_i(x_i, x_{-i})$ is \textbf{ (strictly) concave} in $x_i$ for any fixed $x_{-i}$. In his seminal work, \cite{rosen1965existence} introduced the class of concave games, and showed that every (strictly) concave game has a (unique) Nash equilibrium.\footnote{Concave games are well studied, and possess some other nice properties, see e.g. \cite{ui2008correlated,einy2022strong}.} An important subclass of concave games is the class of \emph{socially-concave games}, introduced by \cite{10.1145/1536414.1536486}. 

\begin{definition}
\label{def:sc}
    A game $G$ is socially-concave if the following properties hold:

    \begin{enumerate}[label=A\arabic*.]
        \item \label{sc:cond1} There exist strictly positive coefficients $\alpha_1, ... \alpha_n > 0$, such that $\sum_{i=1}^n \alpha_i = 1$ and the function $g(x) \coloneqq \sum_{i=1}^n \alpha_i \cdot u_i(x)$ is \textbf{concave} in $x$.
        \item \label{sc:cond2} The utility function of each player $i$ is \textbf{convex} in the actions of all other players. That is, $\forall i \in N, \forall x_i \in X_i$, the function $f(x_{-i}) \coloneqq u_i (x_i, x_{-i})$ is convex in $x_{-i}$.
    \end{enumerate}
\end{definition}

\cite{10.1145/1536414.1536486} showed that every socially-concave game is a concave game, but the reverse direction is not necessarily true. \cite{10.1145/1536414.1536486} also showed that if each player follows any regret minimization procedure in a socially-concave game, then the dynamics are guaranteed to converge. The convergence is in the sense that both the average action vector converges to a Nash equilibrium and the average utility of each player converges to her utility in that Nash equilibrium.


\section{The model}\label{sec: the model}

An $n$-player publishers' game is a game in which $n$ content providers (publishers) generate content (documents) to maximize exposure to users while maintaining the integrity of their original content (initial documents). In this setup, each document is modeled as a $k$-dimensional vector, which can be thought of as the document's \(k\)-dimensional embedding representation. We assume the embedding space is normalized to the $k$-dimensional unit cube $[0,1]^k$. The \(n\) publishers, denoted by the set \(N \coloneqq \{ 1, \dots, n \} \), constitute the set of players of the publishers' game. For any player \(i \in N\), player \(i\)'s set of possible actions in the game is defined to be the embedding space, that is \(X_i \coloneqq [0,1]^k\).

Information needs of the users are denoted by $x^* \in [0,1]^k$ and modeled as vectors in the same embedding space as the publishers' documents. This approach mirrors the common practice in standard models of dense retrieval \cite{zhan2020learning, zhao2022dense}. We model the fact that in real life there are often multiple information needs by a demand distribution \(P^* \in \mathcal{P}([0,1]^k)\), a distribution of information needs. In addition, each publisher has an initial document $x_0^i \in [0,1]^k$.

Distance between two documents in the embedding space is measured by a given semi-metric\footnote{A semi-metric is similar to a metric, except it does not need to satisfy the triangle inequality.} $d: [0,1]^k \times [0,1]^k \to \R_{+}$, which is assumed to be normalized such that for any two documents \(a,b \in [0,1]^k\) we have $ 0 \le d(a,b) \le 1$. Another standard assumption that we make is that \(d(a, x_0^i)\) and \(d(a, x^*)\) are twice differentiable in \(a\) for all the initial documents \(\{x_0^i\}_{i \in N}\) and for every information need \(x^*\).
This assumption is needed for the utilities to be twice differentiable.
Moreover, we assume that $d(a,b)$ is bi-convex, meaning that it is convex in \(a\) for any fixed \(b\) and vice-versa.
The role of \(d\) in our model is two-fold. Firstly, it measures the integrity to the initial content, with the interpretation that a small distance between a publisher's strategy document and her initial document represents strong integrity. Secondly, \(d\) is used by the system designer to assess the relevance of documents to a given information need \(x^*\), with the interpretation that \(d\)-proximity implies relevance.

Publishers' exposure to users is determined by a pre-defined ranking function \(r: [0,1]^{k \cdot n} \times [0,1] ^k \to \mathcal{P}(N) \), selected by the system designer. \(r\) receives as input a strategy profile of documents chosen by the publishers, as well as an information need, and outputs a distribution over the publishers, with the interpretation that \(r_i(x; x^*)\) is the proportion of the users who are interested in the information need \(x^*\) that are exposed to publisher \(i\)'s document if the strategy profile that is played by the publishers is \(x\).\footnote{An alternative interpretation would be that \(r_i(x; x^*)\) is the probability publisher \(i\) would be ranked first in a search engine in response to a query \(x^*\) if the strategy profile that is played by the publishers is \(x\).}
Typically, \(r_i(x; x^*)\) would decrease in \(d(x_i, x^*)\) and increase in \(d(x_j, x^*)\) for \(j \neq i\).\footnote{In addition, ranking functions should be oblivious, meaning they should exhibit symmetry among publishers.}


Each publisher \(i\) tries to achieve two goals simultaneously: on the one hand, maximize the expected chance of her being ranked first by the search engine, which for a given strategy profile \(x\) is \(\E[x^* \sim P^*]{r_i(x; x^*)}\); and on the other hand, provide content \(x_i\) which is as faithful as possible to her initial document, meaning with \(d(x_i, x_0^i)\) as small as possible. Her trade-off between these two goals is determined by an integrity parameter \(\lambda_i > 0\).

Formally, an $n$-player publishers' game is a tuple $G \coloneqq (N, k, d, r, P^*, \{ x_0^i \}_{i \in N}, \{ \lambda_i \}_{i \in N})$. The set of players of the game is \(N \coloneqq \{1 , \dots, n \}\), the action space of each publisher \(i \in N\) is the embedding space $X_i \coloneqq [0,1]^k$, and her utility function is defined as follows:

\begin{equation}
    u_i(x) \coloneqq \E[x^* \sim P^*]{r_i(x ; x^*)} - \lambda_i \cdot d(x_i, x_0^i)
\end{equation}

% We abuse the notations and denote $d^*(x_i) = d(x_i, x^*)$ and $d^0_i(x_i) = d(x_i, x_0^i)$.
We now turn to the natural definition of ranking functions that induce socially-concave games and ranking functions that induce concave games:

\begin{definition}    
We say a ranking function \(r\) induces socially-concave (concave) games if any publishers' game with \(r\) as its ranking function is a socially-concave (concave) game. 
\end{definition}

Note that condition \ref{sc:cond1} of social concavity holds with \(\alpha_i = \frac{1}{n}\) in every publishers' game, since \(\sum_{i=1}^n r_i \equiv 1\). This leads to the following useful lemma, whose proof is deferred to Appendix \ref{app: prrof of lemma r SC iff}.

\begin{lemma}
\label{lemma: r SC iff}
    A ranking function $r$ induces socially-concave games if and only if for every information need \(x^*\), for every publisher $i \in N$ and for every $x_i \in X_i$, $r_i(x_i, x_{-i}; x^*)$ is convex in $x_{-i}$.
\end{lemma}


In the sequel, we restrict our attention to the very natural class of \emph{proportional ranking functions}:

\begin{definition}\label{def: prop}
    We say a ranking function $r$ is a \textbf{proportional ranking function} if there exists a twice differentiable and strictly decreasing function $g:[0,1] \to \R_{++}$ such that
    \begin{equation}
    r_i(x; x^*) = \frac{g \bigl (d(x_i, x^*) \bigr )}{
    \sumj g \bigl (d(x_j, x^*) \bigr )
    }
    \end{equation}
    The function $g$ is called the \textbf{activation function} of $r$.
\end{definition}

Our main objective is to characterize the subset of proportional ranking functions that induce socially-concave games.
These ranking functions possess various desirable properties, such as the existence of a Nash equilibrium, and a guarantee that if publishers engage according to any regret-minimization procedure, they will converge to a Nash equilibrium.
We can then simulate no-regret dynamics for various instances of the publishers' game for different ranking functions, and compare them in terms of publishers' and users' welfare.


\section{Main result}\label{sec: main result}

We now provide a necessary and sufficient condition for a proportional ranking function to induce socially-concave games. This condition turns out to have a relatively simple form: the activation function should be concave.
% We now provide a characterization of the set of all proportional ranking functions that induce socially-concave games. This characterization turns out to have a relatively simple form: a proportional ranking function induces socially-concave games if and only if its activation function is concave.
We show this by proving a stronger statement:

\begin{theorem}
\label{thm: main theorem}
    Let $r$ be a proportional ranking function with activation function $g$. Then, the following are equivalent:
\begin{enumerate}[label=\Roman*.]
        \item\label{II} The activation function \(g\) is concave
        \item\label{III} \(r\) induces concave games
        \item\label{I} \(r\) induces socially-concave games
    \end{enumerate}

    Moreover, if \(d\) is strictly bi-convex, then \(r\) induces strictly concave games if and only if \(g\) is concave.
\end{theorem}

\begin{proof}\label{main proof}
    We prove the theorem by showing that concavity of the activation function is sufficient for social concavity (\(\ref{II} \implies \ref{I}\)), then showing that if \(g\) is not concave then \(r\) does not even induce concave games  (\(\ref{III} \implies \ref{II}\)), which wraps up the proof of the equivalence of \ref{II}, \ref{III} and \ref{I} since \cite{10.1145/1536414.1536486} showed that any socially-concave game is a concave game (\(\ref{I} \implies \ref{III}\)).
    For the moreover part, in Appendix \ref{app: strictly concave} we show that in the case where \(d\) is strictly bi-convex, a concave \(g\) implies that \(r\) induces strictly concave games.

    \underline{\(\ref{II} \implies \ref{I}\):} By Lemma \ref{lemma: r SC iff}, it is enough to show that for every information need \(x^*\), for every publisher $i \in N$ and for every $x_i \in X_i$, $r_i(x_i, x_{-i}; x^*)$ is convex as a function of $x_{-i}$. So let \(i \in N\), \(x^* \in [0,1]^k\), \(x_i \in X_i\).
    Denote \(C=g \bigl (d(x_i, x^*) \bigr )\)
    and \(h(x_{-i}) = \sum_{j \neq i} g \bigl (d(x_j, x^*) \bigr )\).
    So we need to show that the following function is convex in \(x_{-i}\):
    \[
        r_i(x_i, x_{-i} ; x^*)
        = 
        \frac{g \bigl (d(x_i, x^*) \bigr )}{
        \sumj g \bigl (d(x_j, x^*) \bigr ) }
        =
        \frac{C}{C + h(x_{-i})}
    \]

    By our assumption that \(d\) is bi-convex, \(d(x_j, x^*)\) is convex in \(x_j\) for any player \(j \in N\). Since \(g\) is concave and decreasing, \(g \bigl (d(x_j, x^*) \bigr )\) is concave in \(x_j\) as a composition of a concave and decreasing function on a convex function. So \(h(x_{-i})\) is concave in \(x_{-i}\) as a sum of concave functions. 

    Now, define a function \(\ell : \R \to \R\) as follows: \(\ell(t) = \frac{C}{C + t}\). So:

    \[
        r_i(x_i, x_{-i} ; x^*) = \ell \bigl ( h(x_{-i}) \bigr )
    \]

    \(C > 0\) guarantees that \(\ell\) is convex and decreasing in \(\R_+\). Therefore \(r_i(x_i, x_{-i}; x^*)\) is convex in \(x_{-i}\) as a composition of a convex and decreasing function on a concave function. 


    \underline{\(\ref{III} \implies \ref{II}\):} If \(g\) is not concave, there exists \(\hat{a} \in (0,1)\) such that \(g''(\hat{a}) > 0\). We now construct a publishers' game instance \(G\), with \(r\) as its proportional ranking function (with activation \(g\)), which is not a concave game. We construct \(G\) to be a publishers' game with embedding dimension \(k=1\), a number of players \(n\) that satisfies \(n > \frac{2 g'(\hat{a})^2}{g''(\hat{a}) g(0)} + 1\), a one-hot distribution on the information needs that places probability \(1\) on \(x^* = 0\) and a semi-metric \(d(a,b)=|a-b|\). We choose the initial documents of all players \(i \in N\) to be \(x_0^i = 1\).
    Note that since all initial documents are located at \(1\) and the only information need is located at \(0\), the utilities are indeed twice differentiable, as we assume in the sequel.
    Let \(\hat{x}_{-1}\) be a strategy profile of all publishers but publisher \(1\) in which each of the other publishers \(j \neq 1\) plays \(\hat{x}_j = 0\). Now, a simple calculation (deferred to Appendix \ref{app: Derivation of f'' > 0}) shows that the function \(f(x_1) \coloneqq u_1(x_1, \hat{x}_{-1})\) satisfies \(f''(\hat{a}) > 0 \).
    Hence, \(u_1(x_1, \hat{x}_{-1})\) is not concave in \(x_1\), so by definition \(G\) is not a concave game.
\end{proof}

Theorem \ref{thm: main theorem}, together with the findings of \cite{10.1145/1536414.1536486} that in socially-concave games any no-regret dynamics converges, and the guarantee of \cite{rosen1965existence} that (strictly) concave games possess a (unique) NE, leads to the following result:

\begin{corollary}
    Let \(r\) be a proportional ranking function with activation function \(g\). Then, if \(g\) is concave, any no-regret learning dynamics in any publishers' game induced by \(r\) converges. Moreover, any induced publishers' game possesses a NE, and if \(d\) is strictly bi-convex the NE is unique.
\end{corollary}


\section{Experimental comparison of ranking functions}\label{sec: empirical}

In this section, we present some proportional ranking functions with concave activation functions and compare them using no-regret dynamics simulations. 
We highlight that our goal is to study the long-term behavior and dynamics of strategic, rational agents that engage with algorithmic tools for regret minimization, which is different than (and complementary to) other lines of work that evaluate the dynamics of human publishers that may be prone to various biases, e.g. \cite{raifer2017information}.
% When analyzing an SEO environment, the creation of real data using experiments is a challenging task, as discussed in \cite{compSearch}. The process requires construction of ranking systems with our ranking functions, in which publishers will engage in SEO competition while getting feedback from the system in accordance with the selected rating functions. 
Therefore, we chose to evaluate the ranking functions using a code simulation in which agents use the state-of-the-art no-regret algorithm of \cite{Farina2022NearOptimalNL}, which is designated for concave games as in our case.
We compare three families of proportional ranking functions based on some concave and decreasing functions as activation functions.

\begin{itemize}
        \item \textbf{The linear proportional ranking function family}: $g_{lin}(t) = b - t$, where $b>1$ is the intercept hyperparameter.
        \item \textbf{The root proportional ranking function family}: $g_{root}(t) = (1 - t)^a$, where $0 < a < 1$ is the power hyperparameter.
        \item \textbf{The logarithmic proportional ranking function family}: $g_{log}(t) = \ln(c -t)$, where \(c > 2\) is the shift hyperparameter.
\end{itemize}

Let \(r^{lin}\), \(r^{root}\) and \(r^{log}\) be the proportional ranking functions induced by these activation functions. Unless stated otherwise, we use the default values of \(b=1+\delta \), \(a=\frac{1}{2}\), \(c=2+\delta\), where \(\delta \coloneqq 10^{-5}\).
% Let \(r^{lin}\), \(r^{root}\) and \(r^{log}\) be the proportional ranking functions with activation functions \(g_{lin}\), \(g_{root}\) and \(g_{log}\), respectively.


\subsection{Simulation details}\label{subsec: simulation details}

Our simulations utilize the state-of-the-art no-regret algorithm presented in \cite{Farina2022NearOptimalNL}, the Log-Regularized Lifted Optimistic FTRL (hereafter, LRL-OFTRL). For each player, the algorithm uses the current gradient of the utility, the gradients from previous rounds, and a learning rate $\eta$ to decide which action to play in the next round. The important feature of LRL-OFTRL is the logarithmic increase in regret as the dynamics progresses. 
In our simulations, which are carried out in rounds, we define a publishers' game $G$ and let the players choose their action in each round using the LRL-OFTRL algorithm. A simulation is said to \emph{converge} if it has reached an $\varepsilon$-NE. Throughout all simulations, we used homogeneous \(\lambda_i=\lambda \) for all \(i \in N\), the squared Euclidean semi-metric $ d(x,y) = \frac{1}{k} ||x-y||_2^2 $, learning rate \(\eta = 1/2\) and \(\varepsilon=10^{-4}\).
In all simulations, we consider uniform demand distributions over a sample of \(s \in \N\) information needs.\footnote{
Note that while we restrict our simulations to uniform demand distributions, any demand distribution can be approximated with \(s\) large enough. 
}
% In each simulation we draw uniformly i.i.d \(s\) information needs and \(n\) initial documents from the embedding space \([0,1]^k\).

\paragraph{Evaluation criteria} To evaluate the performance of the different ranking functions, we report three evaluation criteria: the publishers' welfare, the users' welfare and the convergence rate. The two welfare measures are defined similarly to previous work \cite{madmon2024search, yao2024rethinking}.
The \emph{publishers' welfare} is defined to be the sum of publisher utilities:

\begin{equation}
    \mathcal{U}(x) \coloneqq \sumi u_i(x) = 1 - \lambda \sumi d^0_i (x_i)
\end{equation}

The \emph{users' welfare} is the expected relevance of the first-ranked document for each information need, where we quantify the relevance of a document $x_i$ by $1-d(x_i, x^*)$, and expectation is taken over both the demand distribution \(P^*\) and the distribution over the publishers \(r(x)\):

\begin{equation}
    \mathcal{V} (x) \coloneqq \E[x^* \sim P^*]{\sumi \bigl(1 - d(x_i, x^*)\bigr) \cdot r_i(x)} = 1 - \E[x^* \sim P^*]{\sumi d(x_i, x^*) \cdot r_i(x)}
\end{equation}

These welfare measures can be evaluated at any strategy profile \(x \in X\), but we report the values obtained in the \(\varepsilon\)-NE the dynamics converged to, as these values represent the \emph{long-term} welfares. The \emph{convergence rate} is simply the number of rounds it took the dynamics to converge. For each parameter configuration and each evaluation criterion, we performed \(500\) simulations, when initial documents and demand distributions were drawn uniformly i.i.d., and constructed bootstrap confidence intervals with a confidence level of 95\% using a bootstrap sample size of $B = 500$.

% \subsection{Ranking functions comparison and hyperparameters effect}
\subsection{Simulations results}

\subsubsection{Comparison between ranking function families}\label{subsec: between}

Figure \ref{fig: lam comp} presents several interesting trends. A prominent phenomenon in the figure is a trade-off between the different measures - whenever an activation function induces an equilibrium in which the publishers' welfare is high, the users' welfare is lower and the game dynamics converge more slowly. 
The activation functions that yield higher publishers' welfare values are the ones that align the ranking function more closely with a uniform ranking (i.e., \(r_i \equiv \frac{1}{n}\)), or, in other words, the ones in which the impact of the publishers' content on the ranking is less significant.
When ranking the documents using these functions, the publishers are less incentivized to create relevant content and thus stay closer to their respective initial documents. This leads to higher publishers' welfare and lower users' welfare. On the contrary, there are less uniform ranking functions, in which the distances from the information needs have a greater influence on the ranking. Those ranking functions encourage publishers to compete for each information need and to generally make their documents more relevant to the users, which leads to higher users' welfare and lower publishers' welfare.\footnote{To elucidate this point, let us compare the activation functions \(g_{lin}\) and \(g_{root}\). Note that \(g_{root}\) is a concave transformation of the linear activation function. When applying a square root to a number in \([0, 1]\), the smaller it is the bigger the factor it is increased by. Therefore, for any fixed profile, the ranking produced by \(g_{root}\) is closer to uniform distribution than that produced by \(g_{lin}\).}
% For instance, when comparing the linear and the root ranking functions it is easy to see that the root activation function is a concave transformation of the linear activation function. When applying a square root to a number in \([0, 1]\) the increase in the value will be relatively bigger as the number decreases. Therefore, for any fixed profile, the ranking induced by the root activation function will be more uniform relative then the ranking induced by the linear activation function.}
In addition, when the ranking functions are less uniform, the absolute values of the gradients increase, which leads to faster convergence. 

In the rest of the section, we demonstrate that this order relation between the ranking functions is robust to changes in the ecosystem structure, such as changes in the game parameters, and show how these changes affect our evaluation criteria. 

\paragraph{The effect of the penalty factor \(\lambda\)}
Figure \ref{fig: lam comp} illustrates how \(\lambda\), the penalty factor, influences our evaluation criteria, showing similar trends to those discussed in \cite{madmon2024search}.
One might expect an increase in \(\lambda\) to harm the publishers' welfare, since a larger \(\lambda\) imposes greater penalty on the publishers for providing content that differs from their initial documents. Yet, a higher \(\lambda\) also incentivizes the publishers to adhere more closely to their initial documents, which increases the publishers' welfare. This two opposing forces explain the non-monotonic trend observed in Figure \ref{fig: lam comp} - for lower values of \(\lambda\), the publishers' welfare decreases as \(\lambda\) increases, until it reaches a minimum point, after which it keeps increasing. The trend in the users' welfare is simpler: it monotonically decreases as $\lambda$ increases, likely because higher penalties lead to less relevant content from publishers. Lastly, there is no significant impact of the penalty factor on the convergence rate.

\begin{figure}
\centering
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{static_figures/lam_comp.png}
\caption{
The effect of the penalty factor \(\lambda\), with $n=3, s=3$ and $k=3$.
% Comparison of the linear, the root and the logarithmic proportional ranking functions across various penalty factor $\lambda$ values, with $n=3$, $s=3$, and $k=3$.
}
\label{fig: lam comp}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{static_figures/n_comp.png}
\caption{The effect of the number of publishers $n$, with $\lambda = 0.5$, $s=3$ and $k=3$. 
}
\label{fig: n comp}
\end{figure}

    
\paragraph{The effect of the number of publishers \(n\)} 
The influence of \(n\) on the welfare measures, as depicted in Figure \ref{fig: n comp}, resembles that of \(\lambda\). Just like \(\lambda\), \(n\) has two opposite effects on the publishers' welfare. On the one hand, higher $n$ values make the competition for top ranking harder, discouraging publishers to participate in it and therefore incentivizing them to stay near their initial documents, thus reducing their penalty factor.
On the other hand, since all publishers incur a penalty, more publishers means more penalties, which directly lowers the publishers' welfare. As a result, the publishers' welfare is not monotonous in $n$ but rather has an internal minimum point. The users' welfare decreases in \(n\) since a bigger \(n\) amplifies publishers' adherence to their initial documents, which makes the content in the corpus less relevant to users.
Lastly, more players result in slower convergence rate, which is not surprising since it is measured by the time taken for the last publisher to reach an $\varepsilon$-NE.

\paragraph{The effect of the demand distribution support size \(s\)} 
As depicted in Figure \ref{fig: s comp}, increasing \(s\) leads to an increase in the publishers' welfare and a decrease in the users' welfare, both trends eventually plateauing. A possible explanation is that when increasing $s$ while fixing $n$, a fixed number of publishers compete for an increasing number of information needs, which makes it harder for the publishers to maximize their exposure. Recall that a publisher's utility from exposure is the expected value of her exposure for different information needs, so when a player is unable to meet a large portion of the information needs, she might be demotivated to try to be relevant to the users and focus on being faithful to her initial document, boosting the publishers' welfare in the expense of the users.

The convergence rate is affected by \(s\) as well. When \(s\) is small, the publishers must compete for the same information needs, which leads to more complicated dynamics and hence to slower convergence. As \(s\) increases, the publishers tend to focus on different information needs (the ones which are the closest to their initial document), therefore we get much simpler dynamics and faster convergence.

\paragraph{The effect of the embedding space dimension \(k\)} Figure \ref{fig: k comp} reveals that while \(k\) has a negligible influence on the publishers' and users' welfare, its effect on the convergence rate is substantial. Specifically, as $k$ increases, the dynamics require more rounds to converge (notice the large scale of the convergence rate axis in Figure \ref{fig: k comp}). In this sense, our dynamics are similar to standard optimization algorithms, where the dimensionality of the problem significantly affects the convergence rate.

\begin{figure}
\centering
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{static_figures/s_comp.png}
\caption{The effect of the demand distribution support size \(s\), with $\lambda = 0.5, n=3$ and $k=3$.}
\label{fig: s comp}
\end{figure}

\begin{figure}
\centering\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{static_figures/k_comp.png}
\caption{The effect of the embedding space dimension $k$, with $\lambda = 0.5$, $n=3$ and $s=3$.
}
\label{fig: k comp}
\end{figure}

\subsubsection{Comparison within ranking function families}
Beyond the comparison between the three ranking function families, tuning the hyperparameters within each family also reveals interesting phenomena. The experimental results supporting these observations are provided in Appendix \ref{ape: hyper comp}, and are discussed here. The results once again underscore the publisher-user trade-off discussed in \S\ref{subsec: between}: hyperparameter values that lead to higher publishers' welfare result in lower users' welfare and slower convergence rate, and vice versa.
As was the case in the comparison between ranking function families, the hyperparameters' values that lead to higher publishers' welfare (and lower users' welfare) are the values that make the ranking function closer to uniform ranking. For example, a decrease in the power parameter \(a\) of \(r^{root}\) can be seen in Figure \ref{fig: root comp} to correlate with an increase in publishers' and a decrease in users' welfare, and indeed when the power parameter \(a\) approaches \(0\), the root proportional ranking function approaches a uniform ranking. That is: \(r^{root}_i \to \frac{1}{n}\) as \(a \to0\). 
Similarly, both the intercept parameter \(b\) of \(r^{lin}\) and the shift parameter \(c\) of \(r^{log}\) are positively correlated with the publishers' welfare and negatively correlated with the users' welfare,
and indeed \(r^{lin}_i \to \frac{1}{n}\) as \(b \to \infty\) and \(r^{log}_i \to \frac{1}{n}\) as \(c \to \infty\).

\section{Discussion}\label{sec: Discussion}

We studied an information retrieval game in which publishers have initial documents they prefer to provide and initiated the analysis of no-regret dynamics in such games. We defined the class of proportional ranking functions, which are ranking functions that are determined by a one-variable scalar activation function, and established a full characterization of which proportional ranking functions induce socially-concave games and which induce concave games. We then used this characterization to conclude that any concave activation function guarantees the convergence of no-regret dynamics, thereby offering a system designer a rich family of ranking functions that, under the assumption that publishers minimize their regret, guarantee the reach of the system to a stable state. We then empirically investigated the publishers' welfare and the users' welfare, as well as the convergence rate, which measures how long it takes the ecosystem to reach stability. In particular, we examined how these three criteria are affected by the choice of the ranking function and by changes in the ecosystem structure.

\paragraph{Limitations} Although we prove convergence of no-regret dynamics whenever the activation function is concave, our approach provides no insights regarding convergence in the case it is not concave. Further, we assumed each publisher is restricted to publishing only one document, while in practice a publisher can write several documents, e.g. in order to compete for exposure from multiple information needs simultaneously. A specific cost function was assumed to capture the cost the publishers incur for deviating from their initial documents.
% Moreover, a specific publisher utility function was assumed (exposure profit minus integrity cost).
A major limitation of our experiments is that we drew \(x_0\) and \(x^*\) i.i.d from a uniform distribution, and the trends presented in our analysis are not guaranteed to hold for other ecosystem distributions. A theoretical welfare and convergence rate analysis are also out of scope. We believe these limitations can serve as interesting directions for future work, and further expand our understanding of the dynamics of strategic publishers.






==> backup.tex <==
% \begin{figure} % Use [p] for positioning the figure on a separate page
%     \centering
%     % First row of figures
%     \begin{subfigure}[b]{width=0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{static_figures/lam_regret_comp.png}
%         \caption{[The effect of the penalty factor \(\lambda\) on the average regret of the publishers, with $n=3, s=3$ and $k=3$.}
%     \end{subfigure}
    
%     \hfill
    
%     \begin{subfigure}[b]{width=0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{static_figures/n_regret_comp.png}
%         \caption{The effect of the number of publishers $n$  on the average regret of the publishers, with $\lambda = 0.5$, $s=3$ and $k=3$.}
%     \end{subfigure}
    
%     \vskip\baselineskip % Vertical space between rows

%     % Second row of figures
%     \begin{subfigure}[b]{width=0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{static_figures/s_regret_comp.png}
%         \caption{The effect of the demand distribution support size \(s\) on the average regret of the publishers, with $\lambda = 0.5, n=3$ and $k=3$.}
%     \end{subfigure}
    
%     \hfill
    
%     \begin{subfigure}[b]{width=0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{static_figures/k_regret_comp.png}
%         \caption{The effect of the embedding space dimension $k$ on the average regret of the publishers, with $\lambda = 0.5$, $n=3$ and $s=3$.}
%     \end{subfigure}

%     \caption{Overall caption for all four figures}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \subfigure[The effect of the penalty factor \(\lambda\) on the average regret of the publishers, with $n=3, s=3$ and $k=3$.]{
%         \includegraphics[width=0.45\textwidth]{static_figures/lam_regret_comp.png}
%     }\label{fig: lam regret}
    
%     \hfill
    
%     \subfigure[The effect of the number of publishers $n$  on the average regret of the publishers, with $\lambda = 0.5$, $s=3$ and $k=3$.]{
%         \includegraphics[width=0.45\textwidth]{static_figures/n_regret_comp.png}
%     }\label{fig: n regret}

% \end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\textwidth,height=\textheight,keepaspectratio]{static_figures/lam_regret_comp.png}
\caption{
The effect of the penalty factor \(\lambda\) on the average regret of the publishers, with $n=3, s=3$ and $k=3$.
}
\label{fig: lam regret}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\textwidth,height=\textheight,keepaspectratio]{static_figures/n_regret_comp.png}
\caption{The effect of the number of publishers $n$  on the average regret of the publishers, with $\lambda = 0.5$, $s=3$ and $k=3$. 
}
\label{fig: n regret}
\end{figure}


\begin{figure}[ht]
\centering
\includegraphics[width=0.5\textwidth,height=\textheight,keepaspectratio]{static_figures/s_regret_comp.png}
\caption{The effect of the demand distribution support size \(s\) on the average regret of the publishers, with $\lambda = 0.5, n=3$ and $k=3$.}
\label{fig: s regret}
\end{figure}


\begin{figure}[ht]
\centering\includegraphics[width=0.5\textwidth,height=\textheight,keepaspectratio]{static_figures/k_regret_comp.png}
\caption{The effect of the embedding space dimension $k$ on the average regret of the publishers, with $\lambda = 0.5$, $n=3$ and $s=3$.
}
\label{fig: k regret}
\end{figure}






















\begin{figure}[ht]
\centering
\includegraphics[width=0.5\textwidth,height=\textheight,keepaspectratio]{static_figures/linear_regret_comp.png}
\caption{The effect of the intercept $b$ on the average regret of the publishers in the linear proportional ranking function, with $\lambda=0.5$, $n=3, s=3$ and $k=3$.}
\label{fig: linear regret}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\textwidth,height=\textheight,keepaspectratio]{static_figures/root_regret_comp.png}
\caption{The effect of the power \(a\) on the average regret of the publishers in the root proportional ranking function, with $\lambda=0.5$, $n=3, s=3$ and $k=3$.}
\label{fig: root regret}
\end{figure}

\begin{figure}[th]
\centering
\includegraphics[width=0.5\textwidth,height=\textheight,keepaspectratio]{static_figures/log_regret_comp.png}
\caption{The effect of the shift \(c\) on the average regret of the publishers in the logarithmic proportional ranking function, with $\lambda=0.5$, $n=3, s=3$ and $k=3$.}
\label{fig: log regret}
\end{figure}





\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{ICLR_2025/figures/uniform_lambda_comparison_no_regret.png}
\caption{The effect of the penalty factor \(\lambda\), when initial documents and demand distributions were drawn uniformly i.i.d. with $n=2, s=1$ and $k=3$.}
\label{fig: uniform baseline}
\end{figure}


\begin{figure}[ht]
    \centering
    % \hspace{5em}
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_-0.5_-0.5_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=-0.5, \; \rho_2=-0.5$}
        \label{fig: normal -0.5 -0.5}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_-0.5_0_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=-0.5, \; \rho_2=0$}
        \label{fig: normal -0.5 0}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_-0.5_0.5_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=-0.5, \; \rho_2=0.5$}
        \label{fig: normal -0.5 0.5}
    \end{minipage}
    % \hspace{5em}

    \vspace{1em}  % space between rows

    % \hspace{5em}
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_0_-0.5_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=0, \; \rho_2=-0.5$}
        \label{fig: normal 0 -0.5}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_0_0_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=0, \; \rho_2=0$}
        \label{fig: normal 0 0}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_0_0.5_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=0, \; \rho_2=0.5$}
        \label{fig: normal 0 0.5}
    \end{minipage}
    % \hspace{5em}

    \vspace{1em}  % space between rows

    % \hspace{5em}
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_0.5_-0.5_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=0.5, \; \rho_2=-0.5$}
        \label{fig: normal 0.5 -0.5}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_0.5_0_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=0.5, \; \rho_2=0$}
        \label{fig: normal 0.5 0}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{ICLR_2025/figures/normal_0.5_0.5_lambda_comparison_no_regret.png}
        \subcaption{$\rho_1=0.5, \; \rho_2=0.5$}
        \label{fig: normal 0.5 0.5}
    \end{minipage}
    % \hspace{5em}
    
    \caption{The effect of the penalty factor \(\lambda\), when initial documents and demand distributions were drawn from a normal distribution with $\rho_1, \rho2 \in \{-0.5, 0, 0.5\}$ and
    $n=2, s=1$ and $k=3$.}
    \label{fig: normal distribution}

\end{figure}




% We consider a different family of instance distributions, on which we compare the proportional ranking functions. In those simulations we focus on the base scenario of $n=2$ and $s=1$. As $s=1$ we can denote the single constant information need by $x^* \in {[0,1]}^k$.
% These distributions diverge from the assumptions of independence between the initial documents and the information need, as well as the assumption of uniform marginal distributions.
% Specifically, we utilize the multivariate truncated normal distribution. For each embedding-space coordinate $j \in [k] = [3]$, the $j$-th entries of the publishers’ initial documents and the information need are sampled from the multivariate truncated normal distribution with mean $(0.5, 0.5, 0.5)$, truncated to $[0,1]^3$, and with the following covariance matrix:

% \[
% \text{Cov} = \begin{array}{c|ccc}
%     & {x_0^1}_j & {x_0^2}_j  & {x^*}_j \\
%     \hline
%     {x_0^1}_j & 1 & \rho_1 & \rho_2 \\
%     {x_0^2}_j & \rho_1 & 1 & \rho_1 \rho_2 \\
%     {x^*}_j & \rho_2 & \rho_1 \rho_2 & 1 \\
% \end{array}
% \]

% Note that while entries in different coordinates remain independent, there is a correlation between the initial documents and the information need within each coordinate.
% When $\rho_1=\rho_2=0$ this corresponds to a truncated multivariate normal distribution with the initial documents and the information need being pairwise independent. 

% The baseline for the distribution comparison is created using the same i.i.d. uniform distribution as was used in \S\ref{sec: empirical}, in order to demonstrate the effect of the penalty factor $\lambda$ while using the proportional ranking functions (we presented similar comparison in \S\ref{subsec: between} but with $n=s=k=3$). Then, we executed the same comparison using the normal multivariate truncated normal distribution, with with $\rho_1, \rho_2 \in \{-0.5,0,0.5\}$. Intuitively, $\rho_1 > 0$ means that the initial documents of the two publishers’ will be closer, and $\rho_2 > 0$, means that publisher $1$’s initial document will be generally closer to the information need. In case of negative $\rho_1$ and $\rho_2$ values, the effect on the documents will be opposite respectively. The publishers' welfare plots are presented in Figure ???, the users' welfare plots are presented in Figure ???, and the convergence' rate plots are presented in Figure ???. It is easy to notice, that for all $3$ measurements, the effects of the initial documents ($x_0$) and the information need ($x^*$) are non significant. The trends discussed in \S\ref{subsec: between} are the same for the different distributions, whose results look almost exactly the same as the results in the baseline figures (???). 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

